Pattern of perturbations from a coherent quantum inflationary horizon

It is proposed that if quantum states of space-time are coherent on null surfaces, holographic Planck-scale fluctuations of inflationary horizons dominate the formation of primordial scalar curvature perturbations. It is shown that the reduction of quantum states on nearly-spherical emergent horizon surfaces around each observer creates a distinctive pattern whose correlations in the angular domain differ from the standard quantum theory of inflation. Causal constraints are used in a semiclassical model to formulate candidate directional symmetries. It is suggested that this hypothesis could provide a physical explanation for several well known anomalies measured in CMB anisotropy. New exact symmetries are predicted, such as a vanishing temperature correlation function at 90 degrees angular separation, that can be tested with current data.

==> rerfereesreports.tex <==
Comments for the editors:

The referee comments were very useful in preparing the revised manuscript.

The referees asked for additional clarity on several issues.

To explain the main differences from the standard picture of inflation, I have added a new section B (and a new figure, Fig. 6) to the Appendix, with specific examples of the physical effect of coherence according to the correspondence with classical gravity. 

To be clearer about the geometrical and causal origin of the candidate symmetries, I have added a new subsection (II.D) and a new figure (now  Fig. 4) which creates a clearer connection between Fig. 3 and Fig. 5.  

The role of cosmic variance has brought up by two of the referees, and I have made changes in the text at several places to clarify this issue. It is actually an interesting point:   there is much less cosmic variance in the holographic predictions than the standard ones, and  the  new symmetries require conspiracies among many harmonics, not just low harmonics, as is often assumed in  models of the anomalies. 
The material now appearing in III.A has been moved, reordered and rewritten from the first version, in order to explain this better.

I have also added several new references, including some theory papers suggested by the referees, and some new measurements that have been reported since the original version was submitted.


RESPONSES TO SPECIFIC COMMENTS FROM REFEREES APPEAR BELOW IN CAPITALS



???????????????????????????
Referee: 1

COMMENTS TO THE AUTHOR(S)
This paper deals with the research line of the so called "holographic inflation". To be more precise, the author proposes that if the inflationary horizon is modeled through holografic quantum gravity, then this imprints on the spectrum of the primordial perturbations some correlations which differ from the standard quantum theory of inflation.

The physical reason is the following. In standard inflation the cosmic perturbations are 
created by quantum fluctuations of the inflaton field vacuum, coupled by linearized 
gravity to the classical background geometry. This picture, according to author, misses completely the highly non perturbative regime of gravity dominating the early universe. In fact, in holographic inflation,  cosmic perturbations are dominated by the holographic degrees of freedom of Planck scale quantum geometry. The fundamental coherence of emergent quantum gravity can imprint symmetries on the causal surfaces, that today can be revealed as relics through particular correlations, in principle observable in the CMB spectrum.

This holographic approach allows to predict new exact symmetries of the perturbations in the angular domain. These in turn could provide physical explanations for several well known anomalies measured in CMB anisotropy.

(a) Perhaps, the author could spend a couple of further sentences, in the Introduction, 
to illustrate why non local quantum correlation coming from holographic quantum 
gravity/geometry should be able to explain what the standard non local quantum 
correlations (which exist also in standard inflation) are not able to explain. 

SOME SENTENCES HAVE BEEN ADDED AS SUGGESTED

The paper is, however, well written and well organized. The predictions, or better, the 
explanations of the major CMB anomalies provided by the holographic quantum gravity inflation appear to be very direct and natural. This is particularly clear in the section III-A, where the classical anomalies of the CMB spectrum are discussed in the light of the (new) holgraphic quantum gravity point of view.

(b) On this point, perhaps, again in Sec.III Points 1-2-3, the paper could gain clarity 
from the insertion of a diagram depicting the prediction of the holographic model, in 
particular for the modes \ell=2, \ell=3, so that also the general reader can compare at 
a glance the new predictions with the observed data of the CMB spectrum.

SINCE THE PREDICTIONS APPEAR IN THE ANGULAR AND NOT THE HARMONIC DOMAIN, THEY ARE NOT APPARENT IN SUCH A FIGURE. THE NEW FIGURE 4 DOES CLARIFY HOW THE SPHERICAL FOOTPRINT LEADS TO THIS

(c) A thing that, in the opinion of this referee, can be improved before going to print, 
is the presentation of the holografic QG approach in the context of other approaches that try to go beyond the standard inflationary model. The effects of quantum gravity on the CMB, in fact, have been evaluated in a number of different approaches, besides that of holografic QG illustrated in the present paper. One quite popular, for example, is the approach through the so called Generalized Uncertainty Principle (GUP), also known as Minimum Length Theories. Papers where this approach to cosmological inflation is discussed are, for example:

A NEW SECTION HAS BEEN ADDED TO THE APPENDIX WITH EXAMPLES OF  THE PHYSICAL EFFECTS OF COHERENT HORIZONS AND THEIR RELATIONSHIP TO SOME OF THESE IDEAS FOR DISCRETENESS AT THE PLANCK SCALE 


A.Chatwin-Davies, A.Kempf, R.T.W.Martin,
"Natural Covariant Planck Scale Cutoffs and the Cosmic Microwave Background Spectrum",
Phys.Rev.Lett. 119, 3, 031301 (2017)
[arXiv:1612.06445 [gr-qc]].

A.Kempf, J.C.Niemeyer, 
"Perturbation spectrum in inflation with cutoff" 
Phys.Rev. D64 (2001) 103501 
[astro-ph/0103225]

F.Scardigli, C.Gruber, P.Chen,
"Black Hole Remnants in the Early Universe",
Phys.Rev.D 83 063507 (2011)
[arXiv:1009.0882 [gr-qc]].

In particular, the last paper shows that the GUP predicts the existence and behavior of 
black hole remnants in the pre inflationary early universe, in a quantity able to imprint 
the cosmological correlations in such a way to explain the quadrupole anomaly of the CMB power spectrum (suppression of the \ell=2 quadrupole mode).

It would be nice if the minor changes described in the above points (a), (b), (c) were 
implemented in the final version of the paper, before going to print.

Referee: 2

COMMENTS TO THE AUTHOR(S)
The author attempts to draw interrelations between "holographic inflation" as hypothesised in a certain way, symmetries imposed based on certain kinds of intuition and geometrical considerations, and observable correlations of curvature perturbations. The author argues that these lead for example to certain constraints on the angular correlation function and other quantities. While the premises are interesting potentially, I have to say I find them somewhat vague, ill-defined and also ad hoc as discussed here. In my opinion these arguments and considerations must be developed somewhat more substantially before concrete statements can be made reliably.

THE ADDED SECTIONS HELP SOMEWHAT TO DEVELOP THE ARGUMENTS MORE FULLY

Referee: 3

COMMENTS TO THE AUTHOR(S)
I think the paper extremely good and of broad interested, as the author claims that using the holographic inflation model, some of the the anomalies presented in the CMB can be explained. I believe the manuscript is suitable for publication on CQG in its present form.  I would have few comments and few question for the authors:

1) On very large-scales  CMB measurements are limited by the cosmic variance, implying that we can
not hope to get enough information  about large scale inhomogeneities from the primary CMB alone, so the prediction of $C_T(90^o)=0$ becomes a challenge.

THE ROLE OF COSMIC VARIANCE IS DIFFERENT IN THIS PICTURE, WHICH IS EXPLAINED BETTER IN THE REVISED SECTIONS

2) Planck collab. has  reported  that quadrupole and octopole are closely aligned. However, they also confirm that this anomaly can also be explained  by using  a scale-dependent dipolar modulation. This model has been studied in detail in recent literature, so this anomaly might be associated to statistical factors.

YES, IT IS ONLY A CANDIDATE SYMMETRY HERE, JUST ONE POSSIBLE EXPLANATION

3) For anisotropic universes, the quadrupole amplitude can be drastically reduced without affecting higher multipoles of the angular power spectrum of the CMB. Is there a way to distinguish the predictions given by these geometries from theories of emergent space-time?

THE ANISOTROPIC UNIVERSES DO NOT LEAD TO THE EXACT ZEROS AND HIGH- MULTIPOLE CONSPIRACIES PREDICTED HERE

4) Because the coherent scalar curvature perturbations on sub-horizon scales, does the tensor-to-scalar ratio remain similar to the one predicted by standard inflationary model?  Can iso-curvature modes or non Gaussian signals emerge from this model?

THE TENSOR MODES ARE MUCH SMALLER IN THIS PICTURE IN RELATION TO THE SCALARS. THERE ARE NO ISOCURVATURE MODES.

Letter reference: DSMo01
